Modeling and Simulation of Reconfigurable Intelligent Surfaces for Hybrid Aerial and Ground-based Vehicular Communications

The requirements of vehicular communications grow with increasing level of automated driving and future applications of intelligent transportation systems (ITS). Beside the ever-increasing need for high capacity radio links, reliability and latency constraints challenge the mobile network supply. While for example the millimeter-wave spectrum and THz-bands offer a vast amount of radio resources, their applicability is limited due to delicate radio channel conditions and signal propagation characteristics. Reconfigurable intelligent surfaces (RISs) as part of smart radio environments (SREs) of future ITS infrastructure promise improved radio link qualities by means of purposeful cultivation of passive reflections. With this, obstructed mmWave or THz beams can be guided around obstacles through RIS reflection paths to improve the otherwise limited coverage. In this article, application use cases of RIS-enhanced vehicular communications are proposed. Beside static deployments of RISs at exterior walls of buildings, unmanned aerial vehicles (UAV) could provide reflection capabilities on demand, while future vehicles could - in a visionary approach - consist of meta-material allowing for their opportunistic utilization within an enriched SRE. Results of a case study based on our multi-scale mobility and network simulation model clearly highlight the potential of RIS deployment for hybrid vehicular communication scenarios. Path loss and outage percentages can be reduced considerably.

==> tex/results.tex <==
\section{Results} \label{sec:results}


==> tex/tables/metrics.tex <==
\renewcommand{\entry}[4]{#1 & #2 & #3 & #4 \\}
\renewcommand{\head}[4]{\toprule \entry{\textbf{#1}}{\textbf{#2}}{\textbf{#3}}{\textbf{#4}}\midrule}
\renewcommand{\cW}{0.4cm}

\aboverulesep = 1pt
\belowrulesep = 1pt

\renewcommand{\baselinestretch}{1.0}

\begin{table}[ht]
	\centering
	\caption{Parameterization of the Transmission Schemes}
	\begin{tabular}{p{2.8cm}|p{\cW}p{\cW}|p{\cW}p{\cW}|p{\cW}p{\cW}}
		
		 & \multicolumn{2}{c|}{\textbf{\mno A}} & \multicolumn{2}{c|}{\textbf{\mno B}} & \multicolumn{2}{c}{\textbf{\mno C}} \\
		\textbf{$\boldsymbol{\Phi}_{\textbf{max}}$} & \textbf{UL} & \textbf{DL} & \textbf{UL} & \textbf{DL} & \textbf{UL} & \textbf{DL} \\
		
		
		
		\toprule
		
		CAT [dB] & 30 & 30 & 30 & 30 & 30 & 30 \\
		pCAT [dB] & 30 & 30 & 30 & 30 & 30 & 30 \\
		ML-CAT [MBit/s] & 30 & 30 & 20 & 50 & 20 & 15 \\
		ML-pCAT [MBit/s] & 30 & 30 & 20 & 50 & 20 & 15 \\
		
		\bottomrule		
		
		
	\end{tabular}

	\label{tab:metrics}
	\vspace{0.1cm}
	\emph{UL}: Uplink, \emph{DL}: Downlink
\end{table}


\ifdefined\singleColumn
	\renewcommand{\baselinestretch}{1.5}
\else
\fi

==> tex/tables/parameters.tex <==
\newcommand{\entry}[2]{&#1 & #2 \\}
\newcommand{\head}[2]{& \toprule \entry{\textbf{#1}}{\textbf{#2}}}

\renewcommand{\baselinestretch}{1}

\begin{table}[ht]
	\centering
	\caption{Validation Parameters}
	\begin{tabular}{p{0.2cm}p{3.5cm}p{3.8cm}}
		\toprule
		\sideHeader{11}{0.5cm}{General} 
		\entry{\textbf{Parameter}}{\textbf{Value}}
		\midrule
		\entry{Data source}{50~kByte/s}
		\entry{Transmission decision interval}{1~Hz}
		\entry{$t_{\min}$}{10~s}
		\entry{$t_{\max}$}{120~s}
		\entry{$\alpha$}{6}
		\entry{$\gamma$ (pCAT)}{2}
		\entry{$\gamma$ (ML-pCAT)}{0.5}
		

		\midrule
		
		\sideHeader{8.5}{0.3cm}{SimuLTE} 
		\entry{Carrier frequency}{$\lbrace900,1800,2100\rbrace$~MHz}
		\entry{Bandwidth}{20~Mhz}
		\entry{\ac{UE} transmission power}{23~dBm}
		\entry{\acs{eNB} transmission power}{43~dBm}
		\entry{Channel model}{WINNER II Urban Macrocell}
		\entry{Other parameters}{\texttt{test\_handover} defaults}

		
		\bottomrule
		
	\end{tabular}
	\label{tab:parameters}
\end{table}

\ifdefined\singleColumn
	\renewcommand{\baselinestretch}{1.5}
\else
\fi


==> tex/tables/throughput.tex <==
\newcommand{\cW}{0.8cm}

\aboverulesep = 1pt
\belowrulesep  = 1pt


\renewcommand{\baselinestretch}{1}

\begin{table*}[ht]
	\centering
	\caption{Coefficient of Determination ($R^2$) for Different Machine Learning Models and Data Aggregation Levels}
	\begin{tabular}{p{0.2cm}p{1cm}|p{\cW}p{\cW}p{\cW}p{\cW}|p{\cW}p{\cW}p{\cW}p{\cW}|p{\cW}p{\cW}p{\cW}p{\cW}p{\cW}}

		& & \multicolumn{4}{c|}{\textbf{\mno A}} & \multicolumn{4}{c|}{\textbf{\mno B}} & \multicolumn{4}{c}{\textbf{\mno C}} \\

		& \textbf{Data} & \textbf{ANN} & \textbf{M5} &\textbf{RF} & \textbf{SVM} & \textbf{ANN} & \textbf{M5} &\textbf{RF} & \textbf{SVM} & \textbf{ANN} & \textbf{M5} &\textbf{RF} & \textbf{SVM} \\
		\toprule	
		\sideHeader{5}{0.5cm}{Uplink} 
		& \textbf{\mno} & 0.685 & 0.754 & \textbf{0.8} & 0.71 & 0.46 & 0.658 & \textbf{0.707} & 0.594 & 0.69 & 0.779 & \textbf{0.82} & 0.728 \\
		& \textbf{Scenario} & 0.729 & 0.779 & \textbf{0.806} & 0.683 & 0.49 & 0.572 & \textbf{0.633} & 0.555 & 0.489 & 0.64 & \textbf{0.686} & 0.572 \\
		& \textbf{eNB} & 0.578 & 0.724 & \textbf{0.731} & 0.592 & 0.285 & 0.432 & \textbf{0.456} & 0.44 & 0.384 & 0.57 & \textbf{0.604} & 0.512 \\
		& \textbf{Cell} & 0.532 & 0.687 & \textbf{0.715} & 0.58 & 0.275 & 0.412 & \textbf{0.444} & 0.397 & 0.355 & \textbf{0.505} & \textbf{0.505} & 0.424 \\
		
		
		\midrule
		\sideHeader{6}{0.5cm}{Downlink} 
		& \textbf{\mno} & 0.499 & 0.603 & 0.591 & \textbf{0.612} & 0.524 & 0.584 & \textbf{0.648} & 0.578 & 0.41 & 0.504 & \textbf{0.552} & 0.531 \\
		& \textbf{Scenario} & 0.551 & 0.62 & 0.615 & \textbf{0.627} & 0.321 & 0.491 & \textbf{0.541} & 0.496 & 0.265 & 0.386 & \textbf{0.422} & 0.41 \\
		& \textbf{eNB} & 0.34 & 0.551 & 0.552 & \textbf{0.58} & 0.263 & 0.317 & 0.357 & \textbf{0.362} & 0.151 & 0.323 & 0.334 & \textbf{0.361} \\
		& \textbf{Cell} & 0.3 & \textbf{0.564} & 0.503 & 0.555 & 0.258 & 0.325 & \textbf{0.379} & 0.372 & 0.19 & 0.296 & \textbf{0.306} & 0.294 \\
	    \bottomrule		
		
	\end{tabular}
	
	\vspace{0.1cm}
	\emph{ANN}: Artificial Neural Network, \emph{M5}: M5 Regression Tree, \emph{RF}: Random Forest, \emph{SVM}: Support Vector Machine 
	\label{tab:throughput}
	\vspace{-0.5cm}
\end{table*}

\ifdefined\singleColumn
	\renewcommand{\baselinestretch}{1.5}
\else
\fi


